Enhancing Privacy in ControlNet and Stable Diffusion via Split Learning

With the emerging trend of large generative models, ControlNet is introduced to enable users to fine-tune pre-trained models with their own data for various use cases. A natural question arises: how can we train ControlNet models while ensuring users' data privacy across distributed devices? Exploring different distributed training schemes, we find conventional federated learning and split learning unsuitable. Instead, we propose a new distributed learning structure that eliminates the need for the server to send gradients back. Through a comprehensive evaluation of existing threats, we discover that in the context of training ControlNet with split learning, most existing attacks are ineffective, except for two mentioned in previous literature. To counter these threats, we leverage the properties of diffusion models and design a new timestep sampling policy during forward processes. We further propose a privacy-preserving activation function and a method to prevent private text prompts from leaving clients, tailored for image generation with diffusion models. Our experimental results demonstrate that our algorithms and systems greatly enhance the efficiency of distributed training for ControlNet while ensuring users' data privacy without compromising image generation quality.

==> resultimages.tex <==
\begin{figure*}[tb]
	\subfigure[Condition]{\includegraphics[width=0.12\linewidth]{figures_more/generated_images/canny/condition/2.png}}
	\subfigure[Centralized]{\includegraphics[width=0.12\linewidth]{figures_more/generated_images/canny/org/2.png}}
	\subfigure[SL]{\includegraphics[width=0.12\linewidth]{figures_more/generated_images/canny/trained/2.png}}
	\subfigure[Ours]{\includegraphics[width=0.12\linewidth]{figures_more/generated_images/canny/autoencoder/2.png}}
	\subfigure[Ours+t]{\includegraphics[width=0.12\linewidth]{figures_more/generated_images/canny/hideprompt/2.png}}
	\subfigure[Ours+c]{\includegraphics[width=0.12\linewidth]{figures_more/generated_images/canny/safe/2.png}}
	\subfigure[Ours++]{\includegraphics[width=0.12\linewidth]{figures_more/generated_images/canny/hidepromptsafe/2.png}}
	\subfigure[LDP rr]{\includegraphics[width=0.12\linewidth]{figures_more/generated_images/canny/dp_rr/2.png}}
	\subfigure[LDP 0.1]{\includegraphics[width=0.12\linewidth]{figures_more/generated_images/canny/dp_gaussian_01/2.png}}
	\subfigure[LDP 0.3]{\includegraphics[width=0.12\linewidth]{figures_more/generated_images/canny/dp_gaussian_03/2.png}}
	\subfigure[LDP 0.5]{\includegraphics[width=0.12\linewidth]{figures_more/generated_images/canny/dp_gaussian_05/2.png}}
	\subfigure[Add 1]{\includegraphics[width=0.12\linewidth]{figures_more/generated_images/canny/addnoise1/2.png}}
	\subfigure[Add 50]{\includegraphics[width=0.12\linewidth]{figures_more/generated_images/canny/addnoise50/2.png}}
	\subfigure[Mixup]{\includegraphics[width=0.12\linewidth]{figures_more/generated_images/canny/mixup/2.png}}
	\subfigure[PS]{\includegraphics[width=0.12\linewidth]{figures_more/generated_images/canny/patchshuffling/2.png}}
	\subfigure[FedAvg]{\includegraphics[width=0.12\linewidth]{figures_more/generated_images/canny/fl/2.png}}
	\caption{\textbf{Image generation:} Images of higher quality means better. Randomly selected and non-cherry-picked examples of images generated with the Canny condition under different methods. The text prompt is \emph{a blue rabbit with glasses}.}
	\label{fig:generation}
\end{figure*}


\begin{figure*}[tb]
	\subfigure[Condition]{\includegraphics[width=0.12\linewidth]{figures_more/generated_images/seg/condition/motor.png}}
	\subfigure[Centralized]{\includegraphics[width=0.12\linewidth]{figures_more/generated_images/seg/org/1.png}}
	\subfigure[SL]{\includegraphics[width=0.12\linewidth]{figures_more/generated_images/seg/trained/1.png}}
	\subfigure[Ours]{\includegraphics[width=0.12\linewidth]{figures_more/generated_images/seg/autoencoder/1.png}}
	\subfigure[Ours+t]{\includegraphics[width=0.12\linewidth]{figures_more/generated_images/seg/hideprompt/1.png}}
	\subfigure[Ours+c]{\includegraphics[width=0.12\linewidth]{figures_more/generated_images/seg/safe/1.png}}
	\subfigure[Ours++]{\includegraphics[width=0.12\linewidth]{figures_more/generated_images/seg/hidepromptsafe/1.png}}
	\subfigure[LDP rr]{\includegraphics[width=0.12\linewidth]{figures_more/generated_images/seg/dp_rr/1.png}}
	\subfigure[LDP 0.1]{\includegraphics[width=0.12\linewidth]{figures_more/generated_images/seg/dp_gaussian_01/1.png}}
	\subfigure[LDP 0.3]{\includegraphics[width=0.12\linewidth]{figures_more/generated_images/seg/dp_gaussian_03/1.png}}
	\subfigure[LDP 0.5]{\includegraphics[width=0.12\linewidth]{figures_more/generated_images/seg/dp_gaussian/1.png}}
	\subfigure[Add 1]{\includegraphics[width=0.12\linewidth]{figures_more/generated_images/seg/addnoise1/1.png}}
	\subfigure[Add 50]{\includegraphics[width=0.12\linewidth]{figures_more/generated_images/seg/addnoise50/1.png}}
	\subfigure[Mixup]{\includegraphics[width=0.12\linewidth]{figures_more/generated_images/seg/mixup/1.png}}
	\subfigure[PS]{\includegraphics[width=0.12\linewidth]{figures_more/generated_images/seg/patchshuffling/1.png}}
	\subfigure[FedAvg]{\includegraphics[width=0.12\linewidth]{figures_more/generated_images/seg/fl/1.png}}
	\caption{\textbf{Image generation:} Images of higher quality means better. Randomly selected and non-cherry-picked examples of generated images with the given condition of Segmentation under different methods. The text prompt is: \emph{a motorcycle}.}
	\label{fig:generationsef}
\end{figure*}

\begin{figure}[tb]
	\subfigure[Condition]{\includegraphics[width=0.24\linewidth]{figures_more/generated_images/scribble/condition/4.png}}\hfill
	\subfigure[Centralized]{\includegraphics[width=0.24\linewidth]{figures_more/generated_images/scribble/org/4.png}}\hfill
	\subfigure[SL]{\includegraphics[width=0.24\linewidth]{figures_more/generated_images/scribble/trained/4.png}}\hfill
	\subfigure[Ours]{\includegraphics[width=0.24\linewidth]{figures_more/generated_images/scribble/safe/4.png}}
	\caption{\textbf{Image generation:} Images of higher quality means better. Randomly selected and non-cherry-picked examples of generated images with the given condition of Scribble. The text prompt is: \emph{a hot air balloon}.}
	\label{fig:generationscribble}
\end{figure}

\begin{figure}[tb]
	\subfigure[Canny]{\includegraphics[width=0.24\linewidth]{figures/reconstruction/canny/celeba/0/condition.png}}\hfill
	\subfigure[SL]{\includegraphics[width=0.24\linewidth]{figures/reconstruction/canny/celeba/0/origin.png}}\hfill
	\subfigure[Ours]{\includegraphics[width=0.24\linewidth]{figures/reconstruction/canny/celeba/0/autoencoder.png}}\hfill
	\subfigure[Ours++]{\includegraphics[width=0.24\linewidth]{figures/reconstruction/canny/celeba/0/safe.png}}\hfill
	\subfigure[LDP rr]{\includegraphics[width=0.24\linewidth]{figures/reconstruction/canny/celeba/0/dp_rr.png}}\hfill
	\subfigure[LDP 0.1]{\includegraphics[width=0.24\linewidth]{figures/reconstruction/canny/celeba/0/dp_gaussian_01.png}}\hfill
	\subfigure[LDP 0.3]{\includegraphics[width=0.24\linewidth]{figures/reconstruction/canny/celeba/0/dp_gaussian_03.png}}\hfill
	\subfigure[LDP 0.5]{\includegraphics[width=0.24\linewidth]{figures/reconstruction/canny/celeba/0/dp_gaussian_05.png}}\hfill
	\subfigure[Add 1]{\includegraphics[width=0.24\linewidth]{figures/reconstruction/canny/celeba/0/add_noise_1.png}}\hfill
	\subfigure[Add 50]{\includegraphics[width=0.24\linewidth]{figures/reconstruction/canny/celeba/0/add_noise_50.png}}\hfill
	\subfigure[Mixup]{\includegraphics[width=0.24\linewidth]{figures/reconstruction/canny/celeba/0/mixup.png}}\hfill
	\subfigure[PS]{\includegraphics[width=0.24\linewidth]{figures/reconstruction/canny/celeba/0/patchshuffling.png}}
		\caption{\textbf{Privacy preserving:} Higher distortion means better privacy preservation. Randomly selected and non-cherry-picked examples of reconstructed condition images by inverse network based attacks when training the ControlNet with condition canny.}
	\label{fig:reconstructionCeleba}
\end{figure}


\begin{figure}[tb]
	\subfigure[Scribble]{\includegraphics[width=0.24\linewidth]{figures/reconstruction/scribble/celeba/condition.png}}\hfill
	\subfigure[Ours]{\includegraphics[width=0.24\linewidth]{figures/reconstruction/scribble/celeba/autoencoder.png}}\hfill
	\subfigure[Scribble]{\includegraphics[width=0.24\linewidth]{figures/reconstruction/scribble/imagenet/condition.png}}\hfill
	\subfigure[Ours]{\includegraphics[width=0.24\linewidth]{figures/reconstruction/scribble/imagenet/autoencoder.png}}\hfill
	\caption{\textbf{Privacy preserving: } Higher distortion means better privacy preservation. Randomly selected and non-cherry-picked examples of reconstructed condition images by inverse network attacks. The condition is scribble. The left two are from CelebA experiments, and the right two are from ImageNet.}
	\label{fig:reconstruction}
\end{figure}
